5G Network Slicing for Wi-Fi Networks

Future networks will pave the way for a myriad of applications with different requirements and Wi-Fi will play an important role in local area networks. This is why network slicing is proposed by 5G networks, allowing to offer multiple logical networks tailored to the different user requirements, over a common infrastructure. However, this is not supported by current Wi-Fi networks. In this paper, we propose a standard-compliant network slicing approach for the radio access segment of Wi-Fi by defining multiple Service Set Identifiers (SSIDs) per Access Point (AP). We present two algorithms, one that assigns resources according to the requirements of slices in a static way, and another that dynamically configures the slices according to the network's conditions and relevant Key Performance Indicators (KPIs). The proposed algorithms were validated through extensive simulations, conducted in the ns-3 network simulator, and complemented by theoretical assessments. The obtained results reveal that the two proposed slicing approaches outperform today's Wi-Fi access technique, reaching lower error probability for bandwidth intensive slices and lower latency for time-critical slices. Simultaneously, the proposed approach is up to 32 times more energy efficient, when considering slices tailored for low-power and low-bandwidth devices, while increasing the overall spectrum efficiency.

==> 5G Network Slicing for Wi-Fi Networks/glossary.tex <==
\pagestyle{empty}

\newglossaryentry{A_B^C}{type=main,name={\ensuremath{A_B^C}},sort=A, description={A dummy symbol }}

%Use \gls{acr} or \glspl{acr} for plural
\newacronym{3gpp}{3GPP}{3rd Generation Partnership Project}
\newacronym{5gppp}{5GPPP}{5G Public Private Partnership}
\newacronym{5qi}{5QI}{5G QoS Identifier}

\newacronym{ack}{ACK}{Acknowledgement}
\newacronym{api}{API}{Application Program Interface}
\newacronym{ap}{AP}{Access Point}
\newacronym{awgn}{AWGN}{Additive White Gaussian Noise}

\newacronym{bssid}{BSSID}{Basic Service Set Identifier}
\newacronym{bss}{BSS}{Basic Service Set}

\newacronym{cca}{CCA}{Clear Channel Assessment}
\newacronym{csma/ca}{CSMA/CA}{Carrier Sensing Multiple Access with Collision Avoidance}
\newacronym{csma}{CSMA}{Carrier Sensing Multiple Access}
\newacronym{cts}{CTS}{Clear to Send}

\newacronym{dcf}{DCF}{Distributed Coordination Function}
\newacronym{difs}{DIFS}{DCF Inter-Frame Spacing}
\newacronym{dl}{DL}{Deep Learning}
\newacronym{dsss}{DSSS}{Direct Sequence Spread Spectrum}

\newacronym{e2e}{E2E}{End-to-End}
\newacronym{edca}{EDCA}{Enhanced Distributed Channel Access}
\newacronym{eirp}{EIRP}{Equivalent Isotropically Radiated Power}
\newacronym{embb}{eMBB}{Enhanced Mobile Broadband}
\newacronym{em}{EM}{Element Management}
\newacronym{epc}{EPC}{Evolved Packet Core}
\newacronym{etsi}{ETSI}{European Telecommunications Standards Institute}

\newacronym{fcs}{FCS}{Frame Check Sequence}

\newacronym{gi}{GI}{Guard Interval}
\newacronym{gui}{GUI}{Graphical User Interface}

\newacronym{ietf}{IETF}{Internet Engineering Task Force}
\newacronym{inp}{InP}{Infrastructure Provider}
\newacronym{iot}{IoT}{Internet of Things}
\newacronym{ism}{ISM}{Industrial Medical Scientific}
\newacronym{itu}{ITU}{International Telecommunication Union}

\newacronym{kpi}{KPI}{Key Performance Indicator}

\newacronym{lan}{LAN}{Local Area Network}

\newacronym{los}{LoS}{Line-of-Sight}

\newacronym{mac}{MAC}{Medium Access Control}
\newacronym{mano}{MANO}{Management and Orchestration}
\newacronym{mcs}{MCS}{Modulation and Coding Scheme}
\newacronym{mimo}{MIMO}{Multiple-Input Multiple-Output}
\newacronym{ml}{ML}{Machine Learning}
\newacronym{mmtc}{mMTC}{Massive Machine-Type Communications}
\newacronym{mpdu}{MPDU}{MAC Protocol Data Unit}
\newacronym{msdu}{MSDU}{MAC Service Data Unit}
\newacronym{mu-mimo}{MU-MIMO}{Multi-User MIMO}

\newacronym{nfvi}{NFVI}{Network Function Virtualization Infrastructure}
\newacronym{nfv}{NFV}{Network Function Virtualization}
\newacronym{nf}{NF}{Network Function}
\newacronym{ngmn}{NGMN}{Next Generation Mobile Networks}
\newacronym{nsi}{NSI}{Network Slice Instance}
\newacronym{ntnu}{NTNU}{Norwegian University of Science and Technology}

\newacronym{ofdma}{OFDMA}{Orthogonal Frequency Division Multiple Access}
\newacronym{ofdm}{OFDM}{Orthogonal Frequency Division Multiplexing}
\newacronym{onf}{ONF}{Open Network Foundation}
\newacronym{os}{OS}{Operating System}

\newacronym{phy}{PHY}{Physical}
\newacronym{psd}{PSD}{Power Spectrum Density}

\newacronym{qoe}{QoE}{Quality of Experience}
\newacronym{qos}{QoS}{Quality of Service}

\newacronym{ran}{RAN}{Radio Access Network}
\newacronym{rl}{RL}{Reinforcement Learning}
\newacronym{rts}{RTS}{Request to Send}
\newacronym{ru}{RU}{Resource Unit}

\newacronym{sdma}{SDMA}{Spatial Division Multiple Access}
\newacronym{sdm}{SDM}{Spatial Division Multiplexing}
\newacronym{sdn}{SDN}{Software Defined Networking}
\newacronym{sdr}{SDR}{Software Defined Radio}
\newacronym{sla}{SLA}{Service Level Agreement}
\newacronym{slo}{SLO}{Service Level Objective}
\newacronym{snr}{SNR}{Signal-to-Noise Ratio}
\newacronym{ssid}{SSID}{Service Set Identifier}
\newacronym{sta}{STA}{Station}

\newacronym{tcp}{TCP}{Transmission Control Protocol}
\newacronym{tpc}{TPC}{Transmit Power Control}

\newacronym{udp}{UDP}{User Datagram Protocol}
\newacronym{ue}{UE}{User Equipment}
\newacronym{urllc}{URLLC}{Ultra-Reliable Low-Latency Communications}

\newacronym{vm}{VM}{Virtual Machine}
\newacronym{vnf}{VNF}{Virtual Network Function}

\newacronym{wdm}{WDM}{Wavelength Division Multiplexing}
\newacronym{wlan}{WLAN}{Wireless Local Area Network}
\newacronym{wsn}{WSN}{Wireless Sensor Network}

